Efficient Approximate Temporal Triangle Counting in Streaming with Predictions

Triangle counting is a fundamental and widely studied problem on static graphs, and recently on temporal graphs, where edges carry information on the timings of the associated events. Streaming processing and resource efficiency are crucial requirements for counting triangles in modern massive temporal graphs, with millions of nodes and up to billions of temporal edges. However, current exact and approximate algorithms are unable to handle large-scale temporal graphs. To fill such a gap, we introduce STEP, a scalable and efficient algorithm to approximate temporal triangle counts from a stream of temporal edges. STEP combines predictions to the number of triangles a temporal edge is involved in, with a simple sampling strategy, leading to scalability, efficiency, and accurate approximation of all eight temporal triangle types simultaneously. We analytically prove that, by using a sublinear amount of memory, STEP obtains unbiased and very accurate estimates. In fact, even noisy predictions can significantly reduce the variance of STEP's estimates. Our extensive experiments on massive temporal graphs with up to billions of edges demonstrate that STEP outputs high-quality estimates and is more efficient than state-of-the-art methods.

==> res/tables/correlation.tex <==
\begin{table}
	\centering
	\caption{Correlation between the top-$K$ edges according to $\totEdgeW(\cdot)$ and the top-$K$ edges according to the temporal min-degree weight $\temporalDeg{\cdot}$. $J_{sim}$ denotes the Jaccard's similarity between the set of the top-$K$ edges according to $\totEdgeW(\cdot)$ and the set of top-$K$ edges according to the $\temporalDeg{\cdot}$ weight. $Spearman_{left}$ denotes the Spearman's coefficient computed considering all the edges in the top-$K$ edges according to the $\totEdgeW(\cdot)$ weight. $Spearman_{inner}$ denotes the Spearman's coefficient computed considering all the edges that are both in the top-$K$ edges according to the $\totEdgeW(\cdot)$ weight and in the top-$K$ edges according to the $\temporalDeg{\cdot}$ weight.}
	\label{tab:correlation}
	\resizebox{\columnwidth}{!}{ 
		\begin{tabular}{llccc}
			\toprule
			$Dataset$ &
			$\delta$ &
			$J_{sim}$ &
			$Spearman_{left}$&
			$Spearman_{inner}$ \\
			\midrule
			\multirow{3}{*}{SO} & $3600s$ & $0.106$ & $0.212$ & $0.129$\\
			& $86400s$ & $0.101$ & $0.141$ & $0.110$ \\
			& $259200s$ & $0.161$ & $0.220$ & $0.186$ \\
			\midrule
			\multirow{3}{*}{BI} & $3600s$ &  $0.251$ & $0.176$ & $0.198$\\
			& $86400s$ & $0.439$ & $0.449$ & $0.353$  \\ 
			& $259200s$ & $0.468$ & $0.509$ & $0.353$ \\
			\midrule
			\multirow{3}{*}{RE} & $3600s$ & $0.297$ & $0.542$ & $0.430$  \\
			& $86400s$ & $0.237$ & $0.424$ & $0.364$  \\ 
			& $259200s$ &$0.268$ & $0.481$ & $0.457$ \\
			\midrule
			\multirow{3}{*}{EC} & $1 \times 10^5 \mu s$ & $0.013$ & $0.151$ & $0.196$ \\
			& $2 \times 10^5 \mu s$ & $0.019$ & $0.179$ & $0.221$ \\
			& $3 \times 10^5 \mu s$ & $0.024$ & $0.215$ & $0.199$ \\
			\bottomrule
		\end{tabular}
	}
\end{table}
